Mixture-Based Correction for Position and Trust Bias in Counterfactual Learning to Rank

In counterfactual learning to rank (CLTR) user interactions are used as a source of supervision. Since user interactions come with bias, an important focus of research in this field lies in developing methods to correct for the bias of interactions. Inverse propensity scoring (IPS) is a popular method suitable for correcting position bias. Affine correction (AC) is a generalization of IPS that corrects for position bias and trust bias. IPS and AC provably remove bias, conditioned on an accurate estimation of the bias parameters. Estimating the bias parameters, in turn, requires an accurate estimation of the relevance probabilities. This cyclic dependency introduces practical limitations in terms of sensitivity, convergence and efficiency. We propose a new correction method for position and trust bias in CLTR in which, unlike the existing methods, the correction does not rely on relevance estimation. Our proposed method, mixture-based correction (MBC), is based on the assumption that the distribution of the CTRs over the items being ranked is a mixture of two distributions: the distribution of CTRs for relevant items and the distribution of CTRs for non-relevant items. We prove that our method is unbiased. The validity of our proof is not conditioned on accurate bias parameter estimation. Our experiments show that MBC, when used in different bias settings and accompanied by different LTR algorithms, outperforms AC, the state-of-the-art method for correcting position and trust bias, in some settings, while performing on par in other settings. Furthermore, MBC is orders of magnitude more efficient than AC in terms of the training time.

==> sections/01-introduction-old.tex <==
% !TEX root = ../2021-clustering-cltr.tex

\section{Old Introduction}
\label{sec:intro} 
% CLTR and bias
\ac{LTR} is the practice of using supervision to train a ranking function.
In traditional \ac{LTR}, explicit relevance labels are used as the supervision source~\citep{liu2009learning}.
In contrast, \ac{CLTR} uses historical interactions such as clicks as the supervision tags for learning to rank the items.
Unlike the costly annotations by human experts, obtaining clicks as implicit feedback incurs no additional cost.
However, the downside of using clicks instead of relevance judgements is \emph{bias}: clicks suffer from different types of bias, such as position bias, selection bias, trust bias, etc.~\citep{joachims2005accurately}.
Generally speaking, bias in clicks means that not all the relevant items have the same chance of being clicked.
For example, position bias means that relevant items at the top of the result list usually absorb more clicks than lower ranked relevant items~\citep{joachims2005accurately};
trust bias means that users trust the search engine and click on higher ranked non-relevant items more than low ranked items~\citep{agarwal2019addressing};
attention bias means that users tend to click more on visually appealing results~\citep{chen2012beyond}; etc.

% debiasing
As a result of bias, the probability of a click is not the same as the probability of relevance.
\emph{Debiasing} is the process of estimating the probability of relevance based on clicks.
In order to have an unbiased ranker, clicks should first be \emph{debiased} before being used in the~\ac{LTR} algorithm~\citep{wang2016learning,joachims2017unbiased}.

% click models and IPS
The relation between the probability of a click and the probability of relevance can be defined by a click model~\citep{chuklin2015click}.
Almost all existing click models build on the \emph{examination hypothesis}, that is, an item is clicked if it is examined and perceived relevant by a user.
In the context of~\ac{CLTR}, to address position bias, the most widely used realization of this hypothesis is:
\begin{equation}
	P(C=1) = P(E=1) \cdot P(R=1),
	\label{eq:intro:positionbias}
\end{equation}
\noindent
where $C$, $E$, and $R$ are binary indicators for click, examination, and relevance, respectively.
It is common in the~\ac{CLTR} literature to assume the~\ac{PBM} for clicks, where $E$ only depends on the item's position.
\citet{joachims2017unbiased} prove that for each click $c = \{0, 1\}$, the value of 
\begin{equation}
	\hat{r} = \frac{c}{P(E=1)}
	\label{eq:intro:ips}
\end{equation}
\noindent
gives an unbiased estimator of relevance.
They call the examination probability $P(E=1)$, \emph{propensity}, and their unbiased method is, hence, called~\ac{IPS}.

% affine
\citet{vardasbi2020when} notice that~\ac{IPS} is not sufficient for debiasing the position and trust bias together.
\ac{IPS} only cares about the relevant clicks, i.e., clicks on the relevant items.
However, in the presence of trust bias, in addition to relevant clicks, non-relevant clicks have to be dealt with as well.
Studies on trust bias reveal that it is not enough to only consider clicks on relevant items; debiasing is not complete without taking into account the clicks over non-relevant items as well~\citep{agarwal2019addressing,vardasbi2020when}.
\citet{vardasbi2020when} introduce an affine correction, a generalization of~\ac{IPS}, which is able to debias both position and trust bias.
The affine correction is based on the following assumption for the click probability:
%
\begin{equation}
	P(C=1) = \alpha \cdot P(R=1) + \beta
	\label{eq:intro:trustbias}
\end{equation}
\noindent
where $\alpha$ and $\beta$ are two position dependent parameters.
When there is trust bias, Eq.~\eqref{eq:intro:trustbias} models the users' click behavior better than Eq.~\eqref{eq:intro:positionbias}, and an unbiased estimate of relevance is given by the affine correction:
\begin{equation}
	\hat{r} = \frac{c - \beta}{\alpha}.
	\label{eq:intro:affine}
\end{equation}
\noindent
% EM problems
Both~\ac{IPS} and its generalization, affine correction, are unbiased provided that the parameters, i.e., $\theta$ in Eq.~\eqref{eq:intro:positionbias} and $\alpha$ and $\beta$ in Eq.~\eqref{eq:intro:trustbias}, are accurately estimated.
In the existing methods, the unbiased~\ac{LTR} problem is solved by simultaneously optimizing two sub-problems\footnote{In this paper it is assumed that no interference in the logging policy is available and we are only given the historical click logs.}:
\begin{enumerate*}
	\item bias parameter estimation for debiasing; and
	\item learning to rank based on the relevance.
\end{enumerate*}
This is done using~\ac{EM} ~\citep{wang2018position,agarwal2019addressing,vardasbi2020when}, or the~\ac{DLA}, which works only for position bias and not for trust bias~\citep{ai2018unbiased}.
Here we focus on the more general case of position and trust bias, so we consider the affine correction with~\ac{EM} for parameter estimation, or~\ac{EM} affine for short.
It is worth noting that our arguments about the affine correction, also holds for the famous~\ac{IPS}, since it is a special case of the affine correction~\citep{vardasbi2020when}.
We distinguish~\ac{EM} affine from oracle affine in which the true values for the parameters are known through an oracle.

Experiments show a gap between the performance of~\ac{EM} affine and oracle affine.
One possible explanation for this gap is that \ac{EM} can trap into the local optimum.
In case of \ac{EM} affine, as we will show in the consequent sections, the error of the estimated relevance is linearly proportional to the error of the estimated bias parameters.
Inaccurate relevance probabilities, in turn, lead to error in the estimated bias parameters in the next Maximization step.
If \ac{EM} were guaranteed to reach a global optimum, these errors would diminish after some iterations.
However, it is known that \ac{EM} converges to local optimum.
Our experiments show the local optimum solution of \ac{EM} affine, differs from the global optimum, given by the oracle affine.
Due to this offset between the performance of \ac{EM} and oracle affine, the former requires substantially more data to converge to the full information case.

\if 0
The second problem stems from the regression-based~\ac{EM}~\citep{wang2018position}.
In regression-based EM, the regression function and LTR algorithm are interactively trained and it is crucial to select the best matching regression function based on the choice for the LTR algorithm.
Furthermore, one has to be concerned with how these two models affect each other: the optimization of the two models are interleaved and any change in one model has an impact on the other.
This dependence, expands the hyper-parameter space.
In other words, in addition to tuning the LTR algorithm, one has to select the best model for the regression function and tune its hyper-parameters.
As there is not a principled way to find the best performing regressor and its hyper-parameters, the only way is to manually tune them over a validation set.
\fi
\mdr{What's the problem? This needs to set us up so that the reader understand why we need a different view point.}

% our intuition
We try to solve this problem by proposing a debiasing method which, unlike the existing methods, acts independently of the LTR part.
% \ac{IPS} and affine are unbiased \ac{LTR}, meaning that they tweak the loss function of an \ac{LTR} algorithm.
The affine correction method is based on the assumption in Eq.~\eqref{eq:intro:trustbias} that marginalizes the click probability by per item relevance probability.
Both the relevance probability $P(R=1 \mid x)$ as well as bias parameters $\alpha_k$ and $\beta_k$ are unknown and estimating each of these quantities depends on the values of the others.
In this paper, we take a different view point.
% Instead of relying on assumptions like Eqs.~\eqref{eq:intro:positionbias} or~\eqref{eq:intro:trustbias}, we propose to consider a mixture model for clicks.
% \im{So what is this different view point exactly? What is new about it? Why is it different? Please discuss all these right away in a couple of sentences.}
% \ali{new: }
We propose to marginalize the distribution of the click count by the per position relevance probability.
With this marginalization, the per position relevance probability is estimated via averaging and the click counts distribution does not depend to the knowledge of per item relevance probability.
In the affine correction, two values representing the probability of clicks over relevant or non-relevant items are learned, whereas in our method, we learn two distributions for the click counts over relevant or non-relevant items.
This change in viewing clicks allows us to separate the debiasing part from the LTR part, and consequently, to solve the mentioned problems with \ac{EM} affine.
Let us elaborate how our method works.
\mdr{These problems need to be mentioned at the end of the previous paragraph: present a problem first, and then propose a solution, instead of the other way around.}
% \begin{enumerate*}
% 	\item requiring too much data to converge; and
% 	\item being sensitive to manual model selection and hyper-parameter tuning.
% \end{enumerate*}

\if 0
According to the~\ac{PBM} assumption, the items at a certain position have the same examination probability, but possibly different relevance probabilities.
Therefore, the difference in the click probabilities of items at a position (corresponding to different queries) comes from their different relevance probabilities.
In other words, looking at a certain position, relevant and non-relevant items have different click probabilities, while two items with the same relevance level have the same click probability.
Therefore, we can model the click probabilities of the items at a certain position by a mixture of two distributions: the relevant clicks and non-relevant clicks distribution.
\fi

% our method
\mdr{Why would be interested in the following separation? Motivate that first.}
In the input of an LTR task, we are interested in distinguishing relevant and non-relevant items.
The debiasing part is responsible for unbiasedly detect the relevant items using the clicks.
A click on an item may be the result of one of the following two disjoint events:
\begin{enumerate*}
	\item a user examined the item and the item was actually relevant; or
	\item the user has examined the item, the item was not relevant, but the user clicked on it anyway due a certain bias, e.g., the trust in a search engine~\citep{agarwal2019addressing} or a visual attractiveness of the item~\cite{chen2012beyond}.
	% \footnote{This case can also involve the accidental clicks}.
\end{enumerate*}
Each event can be indicated by a separate Bernoulli random variable which leads to a binomial distribution for the click count on the item.
Therefore, the distribution of the click count would be a~\emph{mixture} of two binomial distributions.

% mixture-based debiasing
Based on this idea, we propose the~\acfi{MBD} method, which works as follows.
First, for each position in a ranking, a separate mixture model is fitted over the click counts on that position.
% \ali{new: }
In the mixture model, we learn two distributions: one for the click counts over relevant items and another for non-relevant ones.
Then, having learned this mixture and using Bayes' rule, the posterior probability of relevance given click count, is calculated as an estimation of the actual probability of relevance.
Finally, the estimated relevance probabilities are used to produce labels for training a standard~\ac{LTR} algorithm. 
% \im{I would add a bit more details about the proposed method.
% Currently, I can get a good understanding of IPS and the affine correction, but almost no idea how~\OurMethod{} works.}

We prove that the proposed~\OurMethod{} is an unbiased estimator of the probability of relevance and that it has a faster decay in variance compared to the affine correction method.
We also show empirically that~\OurMethod{} converges in performance to the full information case, where manual judgements are used as relevance tags.
% \im{What does ``convergence in performance to the full information case'' mean?}
% Moreover, we analyze the average error and variance of~\OurMethod{} in estimating the relevance and compare it against affine debiasing method.
% \im{And what do we get from this comparison? Is our method better in any way?}
% \ali{new: }
% We show that in the state-of-the-art method, i.e., \citet{vardasbi2020when}'s affine correction method, the error in parameter estimation directly propagates to the error in relevance estimation, while in~\OurMethod{}, due to its indirect dependence, the sensitivity of the relevance estimation to errors in parameter estimation is much lower.
% We note that the main advantage of our mixture-based method, compared to~\ac{IPS} and affine correction, lies in the parameter estimation phase.

% score dist.
% \im{I suggest that we move this paragraph to the discussion section in the end of the paper.}
% \ali{I think it is good to have a brief mention here and move the explanation to the end of the paper.}
\mdr{What exactly is the mixture assumption? Please be precise.}
Our assumption of having a mixture of relevant and non-relevant distributions is related to score distribution models~\todo{ref}.
But \ac{MBD} differs in two important ways.
Unlike scores, clicks are feedback and constitute a source of supervision.
Moreover, a score distribution model is built over the ranked list of items for one query, whereas our mixture model is built over the items at a certain position for different queries.
\if 0
Score distribution models use output scores of a ranker to distinguish the relevant and non-relevant items.
It is assumed that each set of relevant and non-relevant items has a separate score distribution.
Since the ranked list of items is a mixture of relevant and non-relevant items, the score distribution of a ranked list is a mixture of two distributions.
It is worth mentioning that our model and the score distribution models are fundamentally different.
We only share the natural assumption that the items are a mixture of relevant and non-relevant.
One difference between our model and the score distribution model is that, 
Another is that a score distribution model is built over the ranked list of items for one query, whereas our mixture model is built over the items at a certain position for different queries.
% We will discuss more about score distribution models and their fundamental differences to our model in the following sections.
More discussions will come in the later sections.
\fi


% contributions
In summary, our contributions in this paper are:
\begin{enumerate}
	\item We propose a new debiasing method, \acf{MBD}, for removing position and trust bias, and prove its unbiasedness.
	\item We show theoretically that the variance of~\OurMethod{} in estimating relevance decays faster than the state-of-the-art method, i.e., affine correction.
	\item We show experimentally that~\OurMethod{} performs very close to the affine correction with oracle bias parameters, while regression-based EM for affine correction requires substantially more data to reach the same performance as~\OurMethod. 
	We also give a theoretical intuition as to why this happens.
	\if 0
	\item We show experimentally that the performance of regression-based EM depends to the choice of the regression function. \mdr{Why does this matter? And why do we mention this here? Again, go from problem to solution, not the other way around.}
	\ali{Compared to previous points, this is a minor one. We can omit it from here.}
	This dependency is undesirable in general, since it adds to the manual hyper-parameter tuning of the model.
	\OurMethod{} solves this issue, since it is composed of two disjoint parts which can be optimized separately and a change in one part, does not impact the other.
	\fi
\end{enumerate}


\if 0
% user satisfaction
In online search\footnote{or recommendation} services, clicks are usually indicators of user satisfaction~\todo{ref}.
The average number of clicks per session is therefore one of the key factors in evaluating the quality of an online search engine.
Due to contextual factors such as item position, visual aspects, etc. users pay different attention to items in a~\ac{SERP}~\todo{ref}.
\todo{sources of bias}
\im{Is it correct to call those ``contextual factors''?
Where does this terminology come from?
To me, a context is something coming from outside. 
In case of a search system, the document positions, visual information, etc., are all parts of the search system itself, and so I would not call them a context.}

\ali{By context I mean factors outside of the document itself.
So I consider all the factors which affect the clicks either come from inside the document or outside of it.
The former are represented by a single variable: \emph{relevance}.
The latter, I call \emph{contextual}.}
As a consequence, in order to improve the quality of a search engine, it is important to place more interesting items where the users put more attention.

% CLTR
The~\ac{CLTR} problem uses the historical click logs to infer a function that ranks the items based on their interestingness for the users; i.e. relevance.
Unlike traditional~\ac{LTR}, where all the items are examined uniformly by the expert judges, in~\ac{CLTR}, items have different chances of being examined by the users.
Contextual factors, as mentioned earlier, introduce bias in the users behavior.
For example, it is shown in~\citep{joachims2005accurately} that items at higher ranks of a results list consistently absorb more attention than the lower ranked items.
This bias means that clicks are not directly translatable to relevance: they need to be \emph{debiased} first.
Roughly, debiasing means to estimate (unbiased) relevance from the (biased) clicks.
We will give a formal definition later.

% IPS
Earlier works on \emph{unbiased~\ac{LTR}} are based on the examination hypothesis which states that a click is occurred if an item is examined and found attractive by the user~\todo{ref}.
In this case, the click function, i.e. probability of a click in terms of relevance, is a context dependent linear function of relevance and, therefore, the clicks are debiased using a linear transformation, referred by~\ac{IPS}~\citep{wang2016learning,joachims2017unbiased,wang2018position}.

\im{Up to this point, the story is the same as in the first paragraph of the SIGIR short paper.
In that paper, we already worked on the right wording and references, so I suggest to reuse that work here and just rewrite/rephrase what we did in the SIGIR paper.
There, it is a bit too concise, so here we can expand a bit.
Otherwise, the above three paragraphs look a bit wordy and vague to me.}

\ali{Tried hard to be as different as possible to avoid self plagiarism!
Other than that, I tried to argue that it is more reasonable to measure the satisfaction of the user by nDCG@k instead of precision@k, where the re-ranking of top-k results in CLTR does not improve precision@k.}
\todo{top results are important ... [ref]}
\im{I miss the connection between the above general story (IR --> CLTR --> bias --> IPS) and the following paragraph, which discusses such specific (and yet undefined) concepts as ``trust bias'' and ``affine correction/function''. I suggest to add a couple of sentences to better introduce what comes next.}

\ali{The following paragraph is a generalization of its predecessors.
I will add the link.}
\fi


==> sections/figure_tex/severe_bias.tex <==

\begin{table*}[t]
    \caption{Severe bias ($\eta=2$) NDCG@10 comparison of~\OurMethod{} and \ac{AC} on Yahoo! Webscope and MSLR-WEB30k datasets.
    Superscripts $^*$ and $^\dagger$ indicate significance compared to the other correction method with $p<0.01$ and $p<0.1$ respectively.}
    \label{tab:results:severebias}
    \setlength{\tabcolsep}{0.6em}
    \begin{tabular}{l l ccc| ccc}
    \toprule
        &
        & \multicolumn{3}{c|}{Yahoo! Webscope}
        & \multicolumn{3}{|c}{MSLR-WEB30k}
        \\
        \cmidrule(lr){3-5}\cmidrule(lr){6-8} 
        &
        & \bf Bin           & \bf Exp           & \bf Lin          
        & \bf Bin           & \bf Exp           & \bf Lin
        \\
    \midrule
    \multirow{7}{*}{LambdaMART}
    & \multicolumn{5}{l}{\emph{Trained using clicks}}
    \\
    \cmidrule(lr){2-8}
        & No Correction
        & 0.710 & 0.713 & 0.706
        & 0.427 & 0.420 & 0.424
        \\
        & AC
        & 0.722 & 0.718 & 0.732 
        & 0.370 & 0.382 & \bfseries 0.452
        \\
        & \bfseries MBC 
        & \bfseries 0.756\rlap{$^*$} & \bfseries 0.753\rlap{$^*$} & \bfseries 0.746\rlap{$^*$}
        & \bfseries 0.429\rlap{$^*$} & \bfseries 0.438\rlap{$^*$} & 0.451
        \\
        \cmidrule(lr){2-8}
        & \multicolumn{5}{l}{\emph{Trained using oracle knowledge}}
        \\
        \cmidrule(lr){2-8}
        & Ideal-AC
        & 0.746 & 0.718 & 0.739
        & 0.372 & 0.382 & 0.452
        \\
        & Rel. labels
        & 0.759 & 0.757 & 0.763
        & 0.429 & 0.422 & 0.450
        \\
        % & Rel. labels (Grades)
        % & \multicolumn{3}{c}{0.770} & \multicolumn{3}{c|}{0.774}   \\

        \midrule
    \multirow{7}{*}{DNN}
    & \multicolumn{5}{l}{\emph{Trained using clicks}}
    \\
    \cmidrule(lr){2-8}
        & No Correction
        & 0.708 & 0.707 & 0.706
        & 0.393 & 0.397 & 0.397
        \\
        & AC
        & 0.736 & 0.700 & 0.713
        & 0.390 & 0.428 & \bfseries 0.449\rlap{$^*$}
        \\
        & \bfseries MBC 
        & \bfseries 0.742\rlap{$^*$} & \bfseries 0.743\rlap{$^*$} & \bfseries 0.740\rlap{$^*$}
        & \bfseries 0.413\rlap{$^*$} & \bfseries 0.444\rlap{$^*$} & 0.440
        \\
        \cmidrule(lr){2-8}
        & \multicolumn{5}{l}{\emph{Trained using oracle knowledge}}
        \\
        \cmidrule(lr){2-8}
        & Ideal-AC
        & 0.737 & 0.741 & 0.745
        & 0.391 & 0.428 & 0.449
        \\
        & Rel. labels
        & 0.742 & 0.750 & 0.750
        & 0.415 & 0.451 & 0.454
        \\
        % & Rel. labels (Grades)
        % & \multicolumn{3}{c}{} & \multicolumn{3}{c|}{}   \\
        \bottomrule
    \end{tabular}
    \end{table*}
